Reaching the Edge of the Edge: Image Analysis in Space

Satellites have become more widely available due to the reduction in size and cost of their components. As a result, there has been an advent of smaller organizations having the ability to deploy satellites with a variety of data-intensive applications to run on them. One popular application is image analysis to detect, for example, land, ice, clouds, etc. for Earth observation. However, the resource-constrained nature of the devices deployed in satellites creates additional challenges for this resource-intensive application. In this paper, we present our work and lessons-learned on building an Image Processing Unit (IPU) for a satellite. We first investigate the performance of a variety of edge devices (comparing CPU, GPU, TPU, and VPU) for deep-learning-based image processing on satellites. Our goal is to identify devices that can achieve accurate results and are flexible when workload changes while satisfying the power and latency constraints of satellites. Our results demonstrate that hardware accelerators such as ASICs and GPUs are essential for meeting the latency requirements. However, state-of-the-art edge devices with GPUs may draw too much power for deployment on a satellite. Then, we use the findings gained from the performance analysis to guide the development of the IPU module for an upcoming satellite mission. We detail how to integrate such a module into an existing satellite architecture and the software necessary to support various missions utilizing this module.

==> Tables/Coral_breakdown.tex <==
\begin{table*}[t]
    \centering
    
    \begin{tabular}{@{}llrrr@{}}
        \toprule
        & & \multicolumn{3}{c}{Depth multiplier}   \\
        Device & & \multicolumn{1}{c}{0.25} & \multicolumn{1}{c}{0.5} & \multicolumn{1}{c}{1.0}    \\
        \midrule
        \multirow{4}{*}{CoralAI Dev Board Micro}            & Pre-processing  & - & 4153 & - \\
                                                            & Inference & - & 9797 & - \\
                                                            & Pre-processing (memcpy)  & - & 3237 & - \\
                                                            & Inference & - & 9837 & - \\
                                                            \midrule
        \multirow{4}{*}{CoralAI Dev Board Mini}             & Pre-processing & 1517 & 1529 & - \\
                                                            & Inference & 9536 & 10074 & - \\
                                                            & Pre-processing (memcpy) & 227 & 228 & - \\
                                                            & Inference & 9516 & 10057 & - \\
                                                            \midrule
        \multirow{4}{*}{Raspberry Pi + CoralAI TPU}         & Pre-processing & - & 977 & - \\
                                                            & Inference & - & 8514 & - \\
                                                            & Pre-processing (memcpy) & - & 222 & - \\
                                                            & Inference & - & 8551 & - \\
        \bottomrule
    \end{tabular}
    
    \caption{}
    \vspace{-2em}
    \label{tab:coral_breakdown}
\end{table*}

==> Tables/Power_max.tex <==
\begin{table}
    \centering
    \resizebox{\linewidth}{!}{
        {\renewcommand{\arraystretch}{1.25}
            \begin{tabular}{@{}m{10em}R{4.75em}R{4.75em}R{4.75em}@{}}
                \toprule
                & \multicolumn{3}{c}{Depth multiplier}   \\
                & \multicolumn{1}{c}{0.25} & \multicolumn{1}{c}{0.5} & \multicolumn{1}{c}{1.0}        \\
                \cmidrule(lr){2-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}
                \begin{tabular}[t]{@{}c@{}}\\Device\end{tabular}  & \begin{tabular}[t]{@{}c@{}}Power\\draw (mW)\end{tabular} & \begin{tabular}[t]{@{}c@{}}Power\\draw (mW)\end{tabular} & \begin{tabular}[t]{@{}c@{}}Power\\draw (mW)\end{tabular} \\
                \midrule
                Arm Cortex-M7                       &   389   &   N/A     &   N/A     \\
                NVIDIA Jetson Nano, TRT, BS=16  & \textbf{6536} & \textbf{7387} & \textbf{8327}    \\
                Raspberry Pi + NCS2 & 4660 & \textbf{5590} & \textbf{6790} \\
                CoralAI Dev Board Micro & 1560 & 1720 & 2370 \\
                CoralAI Dev Board Mini & 1780 & 2190 & 3380 \\
                Raspberry Pi + CoralAI TPU & 2940 & 3540 & 4570 \\
                \bottomrule
            \end{tabular}
        }
    }
    \caption{Peak power draw of the devices during inference on full-size image. Batch size (BS) of 1 is used if not stated otherwise. The peak power is in bold when exceeding the power budget.}
    \vspace{-1.5em}
    \label{tab:peak_power}
\end{table}

==> Tables/Power_nominal.tex <==
\begin{table*}[t]
    \centering
    
    \begin{tabular}{@{}llrrr@{}}
        \toprule
        & & \multicolumn{3}{c}{Depth multiplier}   \\
        & & \multicolumn{1}{c}{0.25} & \multicolumn{1}{c}{0.5} & \multicolumn{1}{c}{1.0}    \\
        \cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}
        Device  &   & Power draw (mW) & Power draw (mW) & Power draw (mW) \\
        \midrule
        
        \multirow{3}{*}{ARM Cortex-M7}                      & Scenario 1 & - & - & - \\
                                                            & Scenario 2 & - & - & - \\
                                                            & Scenario 3 & 161 & - & - \\
                                                            \midrule
        \multirow{3}{*}{NVIDIA Jetson Nano, TRT, BS=16}     & Scenario 1 & \textbf{2289} & \textbf{3858} & - \\
                                                            & Scenario 2 & 142 & 237 & 526 \\
                                                            & Scenario 3 & 38 & 63 & 140 \\
                                                            \midrule
        \multirow{3}{*}{Raspberry Pi + NCS2}                & Scenario 1 & \textbf{2678} & \textbf{2825} & - \\
                                                            & Scenario 2 & 165 & 174 & 271 \\
                                                            & Scenario 3 & 44 & 46 & 72 \\
                                                            \midrule
        \multirow{3}{*}{CoralAI Dev Board Micro}            & Scenario 1 & - & - & - \\
                                                            & Scenario 2 & 68 & 68 & 92 \\
                                                            & Scenario 3 & 18 & 18 & 24 \\
                                                            \midrule
        \multirow{3}{*}{CoralAI Dev Board Mini}             & Scenario 1 & 1059 & 1165 & - \\
                                                            & Scenario 2 & 65 & 72 & 91 \\
                                                            & Scenario 3 & 17 & 19 & 24 \\
                                                            \midrule
        \multirow{3}{*}{Raspberry Pi + CoralAI TPU}         & Scenario 1 & 1862 & \textbf{2019} & \textbf{2469} \\
                                                            & Scenario 2 & 115 & 124 & 152 \\
                                                            & Scenario 3 & 30 & 33 & 40 \\
        \bottomrule
    \end{tabular}
    
    \caption{Nominal power draw of each device with MobileNetV1 model of different sizes (depth multiplier) for each use case scenario. The combinations of devices and model sizes, which do not fulfil the latency requirements, are omitted as their active duty cycle is greater than 100\%. The power draw is highlighted in bold when exceeding the available power budget.}
    \vspace{-2em}
    \label{tab:nominal_power}
\end{table*}

==> Tables/Results.tex <==
\begin{table*}[t]
    \centering
    
    \begin{tabular}{@{}p{15em}rR{7em}rR{7em}rR{7em}@{}}
    \toprule
        & \multicolumn{6}{c}{Depth multiplier} \\
        & \multicolumn{2}{c}{0.25}             
        & \multicolumn{2}{c}{0.5}              
        & \multicolumn{2}{c}{1.0} \\
        \cmidrule(lr){2-3}
        \cmidrule(lr){4-5}
        \cmidrule(lr){6-7}
    Device 
        & Latency (s)
        & Power consumption (mWh)
        & Latency (s)
        & Power consumption (mWh)
        & Latency (s)
        & Power consumption (mWh) \\
    \midrule
    ARM Cortex-M7 
        & 118.80
        & 12.10
        & N/A 
        & N/A 
        & N/A 
        & N/A \\
    NVIDIA Jetson Nano, TRT, BS=16
        & 1.903          
        & 2.81                       
        & 2.986          
        & 4.73                      
        & 6.036          
        & 10.48  \\
    Raspberry Pi + NCS2 
        & 3.190 %3.604
        & 3.30 %4660mW max, 3710mW avg
        & 3.137 %4.839 
        & 3.48 %5590mW max, 3980mW avg
        & 4.539%8.320
        & 5.44 \\ %6790 max, 4280mW avg
    CoralAI Dev Board Micro
        & 4.880  %$1.220*4$
        & 1.356  %$0.339*4$ %1560mW max, 1000mW avg.% 
        & 5.196  %$1.299*4$ %3236micros buffer, 9780micros inference%
        & 1.360  %$0.340*4$ %1720mW max, 941mW avg.% 
        & 6.031  %$0.965/64*400$ 
        & 1.819 \\  %$0.291/64*400$ \\ %2370mW max, 1090mW avg.% 
    CoralAI Dev Board Mini %idle 4610mW max., 2020mW avg.%
        & 3.902        
        & 1.300 %1780mW max., 1200mW avg.%               
        & 4.118          
        & 1.430 %2190mW max., 1250mW avg%                  
        & 4.667      
        & 1.815   \\  %3380mW max., 1400mW avg%
    Raspberry Pi $+$ CoralAI TPU
        & 3.319       
        & 2.22 %2940mW max., 2480mW avg, 3160 abs max%                 
        & 3.514 %221micros buffer, 8540micros inference%        
        & 2.44 %3540mW max., 2540mW avg, 3990 abs max%                    
        & 4.012
        & 2.93 \\ %4570mW max., 2720mW avg., 4850 abs max%
    \bottomrule
    \end{tabular}
    
    \caption{Latency and power consumption per inference on full-size image with different scaling factors (depth multiplier) of the MobileNetV1 model as measured on corresponding devices. Batch size (BS) of 1 is used if not stated otherwise.}
    \vspace{-1em}
    \label{tab:results}
\end{table*}
